Balanced Clique Computation in Signed Networks: Concepts and Algorithms

Clique is one of the most fundamental models for cohesive subgraph mining in network analysis. Existing clique model mainly focuses on unsigned networks. However, in real world, many applications are modeled as signed networks with positive and negative edges. As the signed networks hold their own properties different from the unsigned networks, the existing clique model is inapplicable for the signed networks. Motivated by this, we propose the balanced clique model that considers the most fundamental and dominant theory, structural balance theory, for signed networks. Following the balanced clique model, we study the maximal balanced clique enumeration problem (MBCE) which computes all the maximal balanced cliques in a given signed network and the maximum balanced clique search problem (MBCS) which computes the balanced clique with maximum size. We show that MBCE problem and MBCS problem are both NP-Hard. For the MBCE problem, a straightforward solution is to treat the signed network as two unsigned networks and leverage the off-the-shelf techniques for unsigned networks. However, such a solution is inefficient for large signed networks. To address this problem, in this paper, we first propose a new maximal balanced clique enumeration algorithm by exploiting the unique properties of signed networks. Based on the new proposed algorithm, we devise two optimization strategies to further improve the efficiency of the enumeration. For the MBCS problem, we propose a new search framework based on search space partition. To further improve the efficiency of the new framework, we propose multiple optimization strategies regarding to redundant search branches and invalid candidates. We conduct extensive experiments on large real datasets. The experimental results demonstrate the efficiency, effectiveness and scalability of our proposed algorithms for MBCE problem and MBCS problem.

==> MaximumBC/conclusion.tex <==
\section{本章小结}
\label{sec:conclusion2}
在本文中，我们研究了签名网络上的最大平衡团搜索问题，该问题被证明是一个NP-难问题。我们首先探索了基于\kw{MBCE}的最大平衡团搜索基础算法。为了克服基础算法中搜索空间过大的问题，我们提出了基于搜索空间划分的搜索算法，每个搜索区域通过对平衡团两侧顶点数量设置不同的下界来细化搜索空间。另外，我们还提出了多种优化策略来进一步减少搜索空间。我们在8个真实数据集上进行了广泛的实验，其中最大的数据集具有上亿条边。实验结果证实了我们提出的算法的高效性、有效性和可拓展性。

==> MaximumBC/implement.tex <==
\section{Implementation} 
%\subsubsection{New Graph Storage Structure}
\label{sec:data}
In the \kw{MBCS} algorithms, through the above analysis, our optimization strategies are lightweight in runtime.  However, the branch pruning strategy and candidate pruning strategy need to apply memory space to build local subgraph for each invocation to get local neighborhood information like $N_{\mathbb{G}_{L(R)}}(v)$ (line 5 of \refalg{color}), $d_{\mathbb{G}}^{+(-)}(v)$ and $N_{\mathbb{G}}^{+(-)}(v)$ (line 2-6 of \refalg{prunev}), and release the memory when algorithms are terminated. Frequent application and release of memory will inevitably lead to the loss of the efficiency. Moreover, another local neighborhood information, i.e., local degree $d_l(v)$ (line 13 of \refalg{fmbcp}, line 14 of \refalg{mbcsp}) is urgent needed in our \kw{MBCE} algorithms and \kw{MBCS} algorithms as well. To solve the memory problem and get local information quickly, in this section, we design a new graph structure that can not only support the \kw{MBCE} algorithms and the \kw{MBCS} algorithms, but also directly provide the local structure information required by our algorithms.

%in this way, the problem of frequent memory application and memory release can be avoided completely. 
%, which are arranged in ascending order according to vertex id. 
For the original graph structure, a signed network $G=(V,E^+,E^-)$ is a combination of two graphs, they are positive graph $G^+=(V,E^+)$ and negative graph $G^-=(V,E^-)$, In $G^+$ and $G^-$, each vertex records their positive neighbors and negative neighbors in adjacency list, respectively. Regarding to the urgent need for the local neighborhood information, we design a new graph structure shown at \reffig{data}. During the search process, for each search branch with $C_L,C_R,P_L, P_R, Q_L,Q_R$, in $G^+$, for each vertex $v$ from $C_L \cup P_L \cup Q_L$, its positive adjacency list $N^+(v)$ is in order of $\{C_L,P_L,None,Q_L\}$, where $None$ presents the positive neighbors of $v$ that do not belong to other sets. Similarly, for each vertex $v$ from $C_R \cup P_R \cup Q_R$, $N^+(v)$ is in order of  $\{C_R,P_R,None,Q_R\}$. $N^-(v)$ is similar with $N^+(v)$. To directly provide the local neighborhood information in current search branch, we use $d_C^{+(-)}(v)$ to indicate the number of $v$'s neighbors in $C_L$ or $C_R$, $d_P^{+(-)}(v)$ to present the number of $v$'s neighbors in $P_L$ or $P_R$,  and $d_Q^{+(-)}(v)$ to record the number of $v$'s neighbors in $Q_L$ or $Q_R$. 
%As $G^+$, $N^-(v)$ is in order of $\{C_R,P_R,None,Q_R\}$ or $\{C_L,P_L,None,Q_L\}$ which depends on the side $v$ belongs to.


Based on the new graph structure, at \refalg{color}, $v$'s local neighbors $N_{\mathbb{G}_{L(R)}}(v)$ correspond to the $P_{L(R)}$ segment of $N^+(v)$. Besides, reconsider \refalg{prunev}, $d^{+(-)}_{\mathbb{G}}(v)$ and $N^{+(-)}_{\mathbb{G}}(v)$ can be directly got by $d_P^{+(-)}(v)$ and $P_{L(R)}$ segment of $N^{+(-)}(v)$, respectively. Moreover, the local degree $d_l(v)$ is supported by $d_P^+(v)+d_P^-(v)+d_Q^+(v)+d_Q^-(v)$ as well. In a result, based on our new graph structure, we can get the needed local information from the graph directly within constant time instead of rebuilding a local subgraph each time, which solves the memory problem in our optimization strategies. 

\begin{example}
For instance, consider the signed network in \reffig{data}, at current search branch,  $C_L=\{v_1\}$, $P_L=\{v_2\}$, $P_R=\{v_3,v_4\}$, $Q_L=\{v_0\}$, our new graph structure is shown at \reffig{data}. In $G^+$, for $N^+(v_0)$, $v_1$ and $v_5$ are $v_0$'s positive neighbors. Since, $v_1$ is in $C_L$, $v_5$ belongs to $None$, $v_0$'s positive adjacency list is $N^+(v)=\{v_1,v_5\}$, $d_C^+(v_0)=1$, $d_P^+(v_0)=0$, $d_Q^+(v_0)=0$. In $G^-$, $v_0$'s negative neighbors are $v_3$ and $v_4$, they are in $P_R$, hence $d_C^-(v_0)=0$, $d_P^-(v_0)=2$, $d_Q^-(v_0)=0$. In a similar way, we can get the adjacency lists of other vertices in the graph.
\end{example}

%(line 21 and line 24 of \refalg{mbcs})
%(line 22 and line 25 of \refalg{mbcs})

\stitle{Maintenance.} Since different search branch has different $C_L,C_R,P_L,P_R, Q_L,Q_R$, the graph structure should be continuously updated as well. Now, we discuss how to maintain the graph structure by considering three update cases: (a)$v$ is added from $P_{L(R)}$ to $C_{L(R)}$; (b)$v$ is removed from $C_{L(R)}$ to $Q_{L(R)}$; (c)current search branch is finished and return to the father search point of the search tree. 
\begin{itemize}
\item For update case(a), given a search state, when add a vertex $v$ from $P_L$ to $C_L$, we update $N^+(u)$ for its positive neighbors $u$, $u\in C_L\cup P_L\cup Q_L$, by moving $v$ from $P_L$ segment to the end of $C_L$ segment, meanwhile, increasing $d_C^+(u)$ by  1, decreasing $d_P^+(u)$ by 1. For $v$'s negative neighbors $u'$, $u'\in C_R\cup P_R\cup Q_R$, we update $N^-(u)$ by moving $v$ from $P_L$ segment to the end of $C_L$ segment, meanwhile, increasing $d_C^-(u')$ by 1, decreasing $d_P^-(u')$ by 1. If move $v$ from $P_R$ to $C_R$, the update procedure is similar with it. 

\item For update case(b), given a search state, when the search from vertex $v$ is finished,  $v$ is moved from $C_L$ to $Q_L$, for its positive neighbors $u$, $u\in C_L\cup P_L\cup Q_L$, we update  $N^+(u)$ by moving  $v$ from $C_L$ segment to the front of $Q_L$ segment, meanwhile, decreasing $d_C^+(u)$ by 1, increasing $d_Q^+(u)$ by 1. For its negative neighbors $u'$, $u'\in C_R\cup P_R\cup Q_R$, we update $N^-(u')$ by moving $v$ from $C_L$ segment to the front of $Q_L$ segment, then we update $d_C^-(u')$ and $d_Q^-(u')$. Besides, if $v$ is removed from $C_R$ to $Q_R$, the update procedure is similar with it.  

\item For update case(c), when current search state is finished, as all vertices in candidate sets are searched, they are in  $Q_L\cup Q_R$ now, we need to recover them to $P_L\cup P_R$ and return to its father search state. In details, for each vertex $v\in Q_L$, for $v$'s positive neighbors $u$, $u\in C_L\cup P_L\cup Q_L$, we update the positive adjacency list of $u$, we recover $v$ from $Q_L$ segment to $P_L$ segment and update $d_P^+(u)$ and $d_Q^+(u)$ respectively. For $v$'s negative neighbors $u'$, $u'\in C_R\cup P_R\cup Q_R$,  we update the negative adjacency list of $u'$, we recover $v$ from $Q_L$ segment to $P_L$ segment, and update $d_P^-(u')$ and $d_Q^-(u')$. For each vertex $v\in Q_R$, the update procedure is similar.
\end{itemize}


\begin{figure}[t]
\begin{center}
\includegraphics[width=0.95\columnwidth]{MaximumBC/fig/datastructure.pdf}
\end{center}
\vspace{-0.2cm}
\topcaption{New graph storage structure}
\label{fig:data}
\vspace{-0.4cm}
\end{figure}



==> MaximumBC/introduction.tex <==

团模型是图数据分析中的一个重要的稠密子图模型。现有的大部分关于团模型的研究都局限于无签名网络，然而，在现实世界中，许多应用场景被建模为由正向边和负向边组成的签名网络。\cite{DBLP:conf/www/ChenY0QY20}提出了基于签名网络的极大平衡团模型，并提出了极大平衡团枚举问题（\kw{MBCE}）来枚举出给定签名网络中的所有极大平衡图。由于\kw{MBCE}的时间开销非常昂贵，使得\cite{DBLP:conf/www/ChenY0QY20}提出的枚举算法难以拓展到大规模签名网络。在本章中，我们研究基于签名网络的最大平衡团问题来寻找顶点数量最多的平衡团。我们证明了该问题是一个NP-难问题。该问题伴随着诸多应用，如社交网络中的对抗社区发现，合作网络中的同领域研究组挖掘，商业联盟搜索，拮抗蛋白质检测等。

在本章中，我们首先探索基于\kw{MBCE}的最大平衡团搜索基础算法。该算法存在搜索空间过大的问题，所以我们又提出了基于搜索空间划分的搜索算法，每个搜索区域通过对平衡团两侧顶点数量设置不同的下界来细化搜索空间。另外，我们还提出了多种优化策略来进一步减少搜索空间。我们在8个真实数据集上进行了广泛的实验，其中最大的数据集具有上亿条边。实验结果证实了我们提出的算法的高效性、有效性和可拓展性。


\section{引言}

% 
图$G=(V,E)$作为一种点和边组成的抽象模型，可以描绘丰富的现实场景，如社交网络、合作网络、通讯网络、时空网络和生物网络等。稠密子图分析是图数据分析中的一个重要的领域，近几十年来，持续吸引着学者们的研究兴趣\cite{luce1949method,DBLP:journals/eor/PattilloYB13,luce1950connectivity,seidman1983network,DBLP:conf/sigmod/BonchiKS19,truss,abello2002massive,pei2005mining,DBLP:journals/pvldb/WangZTT10,DBLP:conf/edbt/ZhouLYLCL12,DBLP:conf/icde/WenQ0CC19}。稠密子图分析主要包括极大稠密子图枚举和最大稠密子图搜索两部分。团(Clique)\cite{luce1949method}模型是最基本的稠密子图模型之一，表示为任意两顶点之间有边连接。最大团表示图中顶点数量最多的团。团模型分析，即极大团枚举问题和最大团搜索问题，在近几年来越来越受到学者们的关注\cite{DBLP:journals/vldb/DasST19,DBLP:conf/icde/LiDWMQY19,DBLP:conf/icde/ZhangZZQY19,DBLP:conf/icde/HuCCSFL19,DBLP:conf/icde/SunWLW17,DBLP:conf/sigmod/ChengKFYZ10,DBLP:journals/pvldb/LuYWZ17,DBLP:conf/aaai/WangCY16,DBLP:conf/aaai/JiangLM17,DBLP:conf/ijcai/CaiL16,DBLP:journals/vldb/Chang20}。极大团枚举问题旨在枚举出图中的所有团，该问题已经被广泛地研究\cite{DBLP:journals/vldb/DasST19,DBLP:conf/icde/LiDWMQY19,DBLP:conf/icde/ZhangZZQY19,DBLP:conf/icde/HuCCSFL19,DBLP:conf/icde/SunWLW17,DBLP:conf/sigmod/ChengKFYZ10}，它可以解决许多应用场景，如寻找社交网络中的交联社区\cite{overlapcommunity}、检测网络层级结构\cite{DBLP:conf/kdd/CreamerRHS07}、在蛋白质交互网络中鉴定蛋白质的复杂程度\cite{protein}。最大团搜索问题旨在搜索出图中顶点数量最大的团，文献\cite{DBLP:journals/pvldb/LuYWZ17,DBLP:conf/aaai/WangCY16,DBLP:conf/aaai/JiangLM17,DBLP:conf/ijcai/CaiL16,DBLP:journals/vldb/Chang20}深入研究了该问题，它可以解决如社交网络上的社区发现\cite{communitydetection}、专家合作网络上的团队检索\cite{DBLP:conf/kdd/LappasLT09}、生物网络中的基因表达和基序发现\cite{Yeger-Lotem5934,motifdiscovery}、复杂网络中的异常检测\cite{emergentclique}等应用。

随着互联网的高速发展，海量的数据带来了新的挑战。图数据变得结构更加复杂，信息更加丰富。在许多场景中，图被刻画成由正边和负边组成的签名网络$G=(V,E^+,E^-)$。结合签名网络中重要的结构平衡理论，\cite{DBLP:conf/www/ChenY0QY20}提出了基于签名网络的平衡团模型，并研究了极大平衡团枚举问题，设计了高效的枚举算法。

然而，对于平衡团模型分析的另一个重要的问题，最大平衡团搜索问题，相关工作仍是一片空白。同时，在签名网络中，极大平衡团的数量往往非常巨大，数量与图中顶点的数量呈指数级关系\cite{DBLP:conf/www/ChenY0QY20}，且极大平衡团之间往往存在许多的重叠部分，使得可以披露的信息量非常有限。另一方面，由于平衡团枚举问题是一个NP-难问题，在签名网络中进行极大平衡团枚举的时间开销非常昂贵，使得它难以在超大规模图数据上进行平衡团枚举。综合以上分析，在本章中，我们致力于解决基于签名网络的最大平衡团搜索问题。极大平衡团枚举的应用在本问题中同样可以得到解决，如社交网络中的对抗社区发现\cite{song2007identifying}，合作网络中的同领域研究组挖掘\cite{DBLP:conf/kdd/LappasLT09}，商业联盟搜索\cite{Margarita2009}，拮抗蛋白质检测\cite{bengal1991functional}等。
最大平衡团搜索问题的规范化定义为：给定一个签名网络$G=(V,E^+,E^-)$，找到$G$中的子图$C_\kw{max}$，使$C_\kw{max}$是一个平衡团同时不存在一个更大的平衡团$C'_\kw{max}$满足$|C'_\kw{max}|>|C_\kw{max}|$。 

% 在\cite{DBLP:conf/www/ChenY0QY20}提出的枚举算法中，一个平衡团表示为$C=\{\}$
% 最大平衡团搜索问题的一个最直接的解决方案是

% 该问题存在以下挑战：
我们在\refsec{preliminaries2}中证明了最大平衡团搜索问题是一个NP-难问题。一个最直接的解决方案是基于\cite{DBLP:conf/www/ChenY0QY20}中提出的极大平衡团枚举算法，通过当前找到的最大平衡团的大小来设置约束条件，使得算法可以找到更大的平衡团，最终得到结果。然而，该解决方案暴露了最大平衡团搜索问题的一个挑战：因为一开始搜索到的平衡团大小往往远小于最终的最大平衡团的大小，如果仅仅通过当前最大平衡团的大小来进行约束，那么算法就需要进行大量的搜索，导致搜索空间过大。所以，我们在本章需要解决的首要任务就是如何有效地减少搜索空间。

% 现有算法

% 我们的主要思想

% \stitle{贡献。}
在本章中，我们做出了以下贡献：


\sstitle{（1）第一个研究最大平衡团模型的工作。}在本章中，我们致力于在给定签名网络中搜索顶点数量最大的平衡团。据我们所知，本工作是首次尝试解决该问题。我们还证明了该问题是一个NP-难问题。

\sstitle{（2）提出了基于搜索空间划分的搜索算法。}为了解决基础算法搜索空间过大的问题，我们提出了基于搜索空间划分的最大平衡团搜索算法。每个搜索区域通过对平衡团两侧顶点数量设置不同的下界来细化搜索空间。当找到比当前最大平衡团更大的平衡团时，我们更新最大平衡团，然后根据最新的最大平衡团大小来提高下一个搜索区域的下界，同时不损失准确性，并最终找到最大平衡团。

\sstitle{（3）设计多种优化策略来提高搜索性能。}我们首先在基础算法的基础上提出了4中可以提前终止搜索的特殊情况。然后，在基于搜索空间划分的搜索算法的基础上提出了候选集剪枝优化策略、图着色剪枝优化策略以及一种全新的数据存储结构。此外，我们还在每一次搜索区域内进行预先边缩减来减少每一轮搜索的签名网络的边规模。我们分析了以上优化策略的时间复杂度，它们都是轻量级优化策略，并在实验中展示了良好的有效性。

\sstitle{（4）在超大规模图数据上进行广泛的性能研究。}我们在真实数据集上进行了广泛的实验研究，其中最大的数据集包含了上亿条边。实验表明，我们的基于搜索空间划分的最大平衡团搜索算法可以高效地在大规模数据集上得到结果，同时搜索区域的数量可以被有效地限制。此外，我们的算法还展现了良好的可拓展性。


% \stitle{文章结构布局。}
关于本章的章节布局，\refsec{preliminaries2}提供了包括极大平衡团模型和问题定义在内的预备知识。\refsec{baseline2}介绍了基础算法。\refsec{spacesplit}介绍了我们基于搜索空间划分的新的搜索算法。\refsec{optimization2}展示了几种优化技术。\refsec{performance2}报告了实验研究的结果。\refsec{conclusion2}总结了本章的工作。


==> MaximumBC/preliminaries.tex <==
%\iffalse
%\bibliography{./reference.bib}
%\fi


\section{问题定义}
\label{sec:preliminaries2}

% In this paper, we consider an undirected and unweighted signed network $G=(V,E^{+},E^-)$, where  denotes the set of vertices, $E^+$ denotes the positive edges and $E^-$ denotes the negative edges connecting the vertices in $G$. We denote the number of vertices and number of edges by $n$ and $m$, respectively, i.e., $n = |V|$ and $m = |E^+| + |E^-|$.  For each vertex $v \in G$, let $N^+_G(v)$ represents the positive neighbors of $v$, i.e, $N^+_G(v) = \{u|(v,u) \in E^+, u,v\in V\}$, and let $N^-_G(v)$ represents the negative neighbors of $v$, i.e, $N^-_G(v) = \{u|(v,u)\in E^-, u,v\in V\}$. We use $d^+_G(v)$ and $d^-_G(v)$ to denote the positive and negative degree of $v$, respectively, i.e., $d^+_G(v) = |N^+_G(v)|$ and $d^-_G(v) = |N^-_G(v)|$. We also use $N_G(v)$ and $d_G(v)$ to denote the neighbors and degree of $v$, i.e., $N_G(v) = N^-_G(v) \cup N^+_G(v)$ and $d_G(v) = d^+_G(v) + d^-_G(v)$. For simplicity, we omit G in the notations if the context is self-evident.
 % We use $n$, $m_p$, $m_n$ to denote the number of nodes and edges in $G$ respectively, i.e, $n = |V(G)|$, $m_p = |E^+(G)$|, $m_n = |E^-(G)|$.

在本章中，对于一个无向无权的签名网络$G=(V,E^{+},E^-)$，我们延续上一章对$n,m,N^+_G(v),N^-_G(v),d^+_G(v),d^-_G(v)$的定义,即$n = |V|$和$m = |E^+| + |E^-|$，对于每个顶点$v \in G$，设$N^+_G(v)$ 表示$v$的正向邻居，即$N^+_G(v) = \{u|(v,u) \in E^+, u,v\in V\}$，让$N^-_G(v)$代表$v$的负邻域，即$N^-_G(v) = \{u|(v,u)\in E^-, u,v\in V\}$。我们使用$d^+_G(v)$和$d^-_G(v)$来表示$v$的正向度数和负向度数，即$d^+_G(v) = |N^+_G(v)|$ 和 $d^-_G(v) = |N^-_G(v)|$。我们还用$N_G(v)$ 和 $d_G(v)$ 表示$v$的邻居和度数，即$N_G(v) = N^-_G(v) \cup N^+_G(v)$和$d_G(v) = d^+_G(v) + d^-_G(v)$。为了直观起见，在下文中我们省略以上符号中的$G$。

我们首先回顾极大平衡团的定义：

\begin{definition}
\label{def:balancecommunity}
\textbf{(极大平衡团)} 给定一个签名网络$G=(V,E^{+},E^-)$, 一个极大平衡团$C$ 是$G$中的一个极大子图，并且满足以下要求:
\begin{itemize}
	\item 完全性: $C$是完全的, 即, $\forall u,v \in C \rightarrow (u,v)\in E^+ \cup E^-$。
	\item 平衡性: $C$是平衡的, 即, 它可以被分成两个子图$C_L$ 和 $C_R$, 使得 $\forall u,v\in C_L$ 或 $u,v \in C_R   \rightarrow (u,v) \in E^+$, 并且 $\forall u\in C_L, v \in C_R$ 或 $u\in C_R, v \in C_L  \rightarrow (u,v) \in E^-$。%\item Maximal: There doesn't exist any sub-network $C'$ such that $C'$ is a balanced clique and $C \subseteq C'$.
\end{itemize}
\end{definition}
在本章中，我们主要研究最大平衡团， 用$C_{\kw{max}}$表示，定义如下：
\begin{definition}
\label{def:maximumbc}
\textbf{(最大平衡团)} 给定一个签名网络$G=(V,E^{+},E^-)$, 一个最大平衡团$C_{\kw{max}}$ 是$G$中的一个极大子图，并且满足以下要求:
\begin{itemize}
    \item $C_{\kw{max}}$是一个极大平衡团。
    \item $C_{\kw{max}}$是最大的，即不会存在任何一个极大平衡团 $C'$ 使得$|C_{\kw{max}}|<|C'|$。
\end{itemize}
\end{definition}


对于一个最大平衡团$C_{\kw{max}}=\{C_L,C_R\}$，我们用$\epsilon$表示我们用$C_{\kw{max}}$中顶点的数量，即$\epsilon=|C_L|+|C_R|$。 在本章中，我们的目的是在给定的签名网络中寻找最大平衡团。由于许多实际应用要求$C_L$ 和 $C_R$ 中的顶点数不小于一个固定的阈值，我们保留对$|C_L|$ 和 $|C_R|$的大小约束$k$，也就是说，最大平衡团需要满足$\underline{\epsilon} \geq k$。我们将需要解决的问题归纳如下：
% $\overline{\epsilon}$表示$C_L,C_R$中较大的一边的顶点数量，即$\overline{\epsilon}=max\{|C_L|,|C_R|\}$。相似地，我们用$\underline{\epsilon}$表示$C_L,C_R$中较小的一边的顶点数量，即$\underline{\epsilon}=min\{|C_L|,|C_R|\}$。


\stitle{问题定义。} 给定一个签名网络 $G$ 和 大小阈值$k$， 最大平衡团搜索问题（\underline{M}aximum \underline{B}alanced \underline{C}lique \underline{S}earching(\kw{MBCS})） 将寻找出$G$中的最大平衡团 $C_\kw{max}$ 使得$C_\kw{max}$ 的顶点数量最多，同时满足单侧顶点数量$\geq k$。

\begin{figure}
\begin{center}
\begin{tabular}[t]{c}
 \includegraphics[width=0.65\columnwidth]{MaximumBC/fig/example1.pdf}
\end{tabular}
\end{center}
\vspace{-0cm}
\topcaption{签名网络$G$中的最大平衡团$C_\kw{max}$ ($k=2$)}
\label{fig:cmax}
\vspace{-0cm}
\end{figure}

\begin{example}
\label{exp:preliminary2}
如\reffig{cmax}所示，$G$是一个签名网络，其中正向边由实边表示，负向边由虚边表示。假设$k$ = 2，根据最大平衡团的定义，$G$中的最大平衡团$C_\kw{max}=\{\{v_0,v_1,v_3\},\{v_5,v_6,v_7\}\}$。$G$中不存在比$C_\kw{max}$更大的平衡团。
\end{example}

% \stitle{问题难点。} \kw{MBCS}问题是一个NP-难问题。在上一章中，我们已经证明了极大平衡团枚举问题是一个难问题。给定一个签名网络$G$和大小阈值$k$，$G$中只存在一个极大平衡团满足$k$的大小约束，那么在$G$上的极大平衡团就是$G$中最大平衡团，在$G$中进行极大平衡团的枚举过程等同于最大平衡团搜索过程，又因为极大平衡团枚举问题已经被证明是一个NP-难问题，所以我们的最大平衡团搜索问题也是一个NP-难问题。
\stitle{问题难点。} \kw{MBCS}问题是一个NP-难问题。与极大平衡团枚举问题的NP-难性证明类似，给定一个普通图$G(V,E)$，我们现在转化$G$为一个签名网络$G'$，$G$中的边全部转化为$G'$中的正向边。然后，向$G'$添加一个顶点$v$，同时$v$与$G'$中的所有顶点都有负向边连接。当$k$=1时，$G$中的最大团$C$对应了$G'$中的最大平衡团$C'$，$C'=\{C,\{v\}\}$。那么在签名网络中的最大平衡团搜索问题就可以规约为无签名网络上的最大团搜索问题。后者已经被证明是一个NP-难问题\cite{approxiclique1}，所以我们的问题也是一个NP-难问题。





==> MaximumBC/related.tex <==
\section{相关工作}
\label{sec:related}

\stitle{签名网络分析。}今年来，签名网络分析引起了广泛的关注。在这些工作中，解释签名网络中潜在社会演化过程的理论得到了广泛的研究。在这些理论中，\emph{结构平衡理论(structural balance theory)}是最基本、最主要的理论 \cite{zheng2015social}。结构平衡理论最初是在\cite{heider1946attitudes}中引入的，并在\cite{harary1953notion,cartwright1956structural}中推广。之后，结构平衡理论得到了广泛的发展\cite{marvel2009energy,abell2009structural,leskovec2010signed,marvel2011continuous,derr2018signed}。在这些著作中，值得一提的是，\cite{marvel2011continuous}的作者对签名网络的演化过程进行了建模，并从理论上证明了当顶点间初始友好度的均值$\mu \leq 0$时，网络将演化为一个平衡团。\cite{zheng2015social}对结构平衡理论进行了全面综述。

除了签名网络的相关理论，在签名网络上进行信息挖掘也发表了大量的文献。其中，与我们最密切相关的工作是\cite{li2018efficient}，它提出了$(\alpha,k)$-团模型。给定一个有符号网络$G$，$(\alpha,k)$-团被定义为一个极大团$C$，使得$C$中每个顶点的负向度数不大于$k$，$C$中每个顶点的正向度数不小于$\alpha k$。与我们的模型相比，$(\alpha,k)$-团模型只考虑了团的正负边数量，完全忽略了团的结构平衡性，这使得$(\alpha,k)$-团模型与我们的模型有本质的不同。另一个相关工作是\cite{hao2014detecting}，它提出了一个$k$-平衡可信团模型。一个$k$-平衡可信团（$k$-balanced trusted clique）被定义为一个包含$k$个顶点的团，团中的边全部由正边组成。虽然$k$-平衡可信团模型与我们的模型有相似的名称，但它忽略了集团中的负边，这意味着它完全忽略了负边的信息。

% \stitle{Signed network analysis.} Signed network analysis has attracted much attention in the literature. In these works, the theories explaining the potential social dynamics process in signed networks have been extensively studied. Among these theories, \emph{structural balance theory} is the most fundamental and dominant one \cite{zheng2015social}. Structural balance theory is originally introduced in \cite{heider1946attitudes} and generalized in the graph  formation in \cite{harary1953notion,cartwright1956structural}. After that, structural balance theory is developed extensively \cite{marvel2009energy,abell2009structural,leskovec2010signed,marvel2011continuous,derr2018signed}. In these works,  it is interesting to mention that the authors in \cite{marvel2011continuous} model the evolving procedure of a signed network and theoretically prove that the network would evolve into a balanced clique when the  mean value of the initial friendliness among the vertices $\mu \leq 0$. \cite{zheng2015social} provides a comprehensive survey on structural balanced theory.

% Besides theories on signed networks, a large body of literature on mining signed networks has been emerged.  Among them, the most closely related work to ours  is \cite{li2018efficient} in which an $(\alpha, k)$-clique model is proposed. Given a signed network $G$, an $(\alpha, k)$-clique is defined as a maximal clique $C$ such that the negative degree for each vertex in $C$ is not greater than $k$ and the positive degree for each vertex in $C$ is not less than $\alpha k$. Compared with our model,  $(\alpha, k)$-clique model only considers the amount of positive and negative edges in the clique and the structural balance of the clique is totally ignored, which makes $(\alpha, k)$-clique model essentially different from our model. In \cite{hao2014detecting}, a $k$-balanced trusted clique model is proposed. A $k$-balanced trusted clique is defined as a clique with $k$ vertices consisting with positive edges only. Although the $k$-balanced trusted clique model has a similar name with our model, it ignores the negative edges in the clique, which means the information of the negative edges are totally missed.

签名网络中的社区检索也与我们的工作有关。例如，\cite{gao2016detecting,lo2011mining,chu2016finding,nature2017,DBLP:journals/jmlr/LiuTM17,DBLP:journals/pami/LiuXTZ19}的目的是寻找签名网络中的对抗社区。这些工作主要集中在探索几组稠密子图，其中在大多数工作中都没有一个清晰的社区模型的结构定义，而我们的工作是枚举签名网络中的极大平衡团结构。此外，这些算法通常涉及复杂的优化过程，因此很难处理大型签名网络，而我们提出的算法可以扩展到在数亿条边的大型签名网络中枚举所有的极大平衡团。更多有关签名网络挖掘的调查可在\cite{tang2016survey}中找到。

% Community detection in signed networks is also related to our work. For example, \cite{gao2016detecting,lo2011mining,chu2016finding,nature2017,DBLP:journals/jmlr/LiuTM17,DBLP:journals/pami/LiuXTZ19} 
% aim to find the antagonistic communities in a signed network. These works mainly focus on exploring several groups of dense subgraphs and most of them don't have a clear structural definition of their community model, while our work aims to enumerate the clique structure in a signed network. Moreover, these solutions generally involve a complicated optimization procedure, thereby, they are hard to handle large signed networks, while our proposed algorithm is scalable to enumerate all the maximal balanced cliques in large signed networks with hundreds of millions of edges as verified in our experiments. A  survey on signed network mining can be found in \cite{tang2016survey}.
% partitioning the signed network into several dense subgraphs

%presents $(\epsilon, min_{size})$-$rQAC$ model which has a bi-quasi-clique formed of negative edges between communities. \cite{} presents a $DAC$ model which has a negative bi-clique between communities. Both of above models ignore the cohesiveness of positive edges within communities, i.e., each community only need to be a CC or SCC formed of positive edges, which is vary sparse. \cite{chu2016finding} are signed community mining methods of data mining, aiming to find multiple antagonistic communities, while our work aims to find cliques in signed networks, moreover, they cannot handle large scale networks due to expensive time complexity of data mining method.

% \stitle{Clique on unsigned networks.} Clique model is one of the most fundamental cohesive subgraph models. \cite{bron1973finding} proposes an efficient algorithm for maximal clique enumeration based on backtracking search.\cite{R2}  first considers the memory consumption during the maximal clique enumeration. Based on \cite{bron1973finding}, more efficient algorithms for maximal clique enumeration are investigated \cite{tomita2006worst,eppstein2010listing,eppstein2011listing}.\cite{eppstein2010listing} proposes a novel branch pruning strategy, pivot pruning, which can efficiently reduce the search space by ignoring the search process from the neighbors of the pivot. \cite{zhang2014finding} studies the maximal biclique enumeration problem on bipartite graphs.\cite{zhang2014finding} keeps growing the vertex set in one side and peeling the vertex set in another side to enumerate the maximal biciques.  It also utilizes some techniques to further improve the enumeration performance, such as choosing vertex with small degree from candidate set to reduce the search tree depth and pruning vertices which may produce non-maximal bicliques. These techniques for biclique enumeration inspire our techniques presented in \refsec{localpruning}.

\stitle{无签名网络上的团模型。}团模型是最基本的稠密子图模型之一。\cite{bron1973finding}提出了一种基于回溯搜索的极大团枚举算法。\cite{R2}  最先在团枚举过程中考虑了内存消耗。基于\cite{bron1973finding}，更多有效的最大团枚举算法被提出来\cite{tomita2006worst,eppstein210listing,eppstein2011listing}，\cite{eppstein2010listing}提出了一种新的分支剪枝策略：中心点修剪（pivot prunning），该策略通过忽略中心点邻居的搜索过程，有效地减少了搜索空间。\cite{zhang2014finding}研究了二分图上的极大双团（bi-clique）的枚举问题。\cite{zhang2014finding}通过不断增长一边的顶点集，剥去另一边的顶点集来枚举最大双团数。它还利用了一些技术来进一步提高枚举性能，如从候选集中选择度较小的顶点来减少搜索树的深度，以及对可能产生非极大双团的顶点进行剪枝。这些双团枚举技术启发了\refsec{localpruning}中介绍的技术。

%In our work, we modify these optimizations to be available for finding maximal balanced cliques in signed networks. However, there are many differences between our techniques and [38]. For details, \cite{zhang2014finding} considers single vertex which can be directly added into current biclique from candidate set. In this way, the current search branch can not be early terminated directly. In the ET Rule 3 of our paper, we consider whether all vertices in the candidate set can form an exact maximal balanced clique with current result together, if so, we can terminate the search branch directly.}

\cite{fakhfakh2017algorithms}回顾了最近在最大团枚举方面的进展。基于团，其他稠密子图模型最近也引起关注，如$k$-core\cite{seidman1983network}，$k$-truss\cite{A6,DBLP:conf/sigmod/HuangCQTY14}，$k$-edge connected component\cite{A7,DBLP:journals/pvldb/YuanQLCZ16,DBLP:journals/vldb/YuanQLCZ17}，$(r,s)$-nucleies\cite{Sariyuce2015finding,DBLP:journals/tweb/SariyuceSPC17}。 值得注意的是，我们的平衡团模型不同于现有的无签名网络上的稠密子图模型，现有的工作不能很好地解决我们的问题。如果只考虑签名网络中的正边，采用传统的无签名网络的稠密子图搜索方法，发现的结果会忽略负边，使之丢失签名网络中的关于负边的一半的有意义信息。

% \cite{fakhfakh2017algorithms} reviews recently advances in maximal clique enumeration.  Based on clique, other cohesive subgraph models are also studied recently, such as $k$-core \cite{seidman1983network}, $k$-truss\cite{A6,DBLP:conf/sigmod/HuangCQTY14}, $k$-edge connected component\cite{A7,DBLP:journals/pvldb/YuanQLCZ16,DBLP:journals/vldb/YuanQLCZ17}, $(r, s)$-nuclei \cite{sariyuce2015finding,DBLP:journals/tweb/SariyuceSPC17}. Note that our balanced clique model is different from the existing cohesive subgraph models on unsigned networks and it cannot be well solved by the existing works. If we just consider the positive edge in the signed network and use the traditional methods on unsigned networks for community detection, the found results would  ignore the negative edges and half meaningful information in the signed network is lost.

%To the best of our knowledge, the balanced clique model proposed in this paper is the first clique model considering the structural balance in signed networks.%


==> extensions.tex <==
\section{Extension}
\label{sec:extensions}
Our techniques can be extended to support the maximal balanced clique enumeration upon external-memory computation paradigm.% and parallel computation paradigm.

\stitle{External-memory \kw{MBCE}.} In external-memory computation paradigm, the size of the main memory is limited, which leads to the input signed network cannot fit in the main memory. Thus, external-memory \kw{MBCE} aims to enumerate the maximal balanced cliques with as few I/Os as possible when $G$ is stored on the disk.

Let $S_i$ be a set of vertices in $G$.  For $S_i$, the 1-hop neighbor subgraph of $S_i$ is the subgraph $G'_i$ of $G$  induced by the vertices in $S_i$ together with their 1-hop neighbors. Since the diameter of a maximal balanced clique is 1, for  $S_i$, we can guarantee that the maximal balanced cliques that have at least a vertex in $S_i$ are contained in $G'_i$, which means we can enumerate the maximal balanced cliques related to $S_i$ locally based on $G'_i$. Therefore,  we first partition the vertices of $G$ into several sets $S_1, S_2, \dots, S_t$ such that the 1-hop neighbor subgraph of $S_i$ can be fitted in the main memory. Then, for each subgraph $G'_i$, we enumerate the maximal balanced cliques in $G'_i$ with our proposed in-memory algorithm. The only remaining problem is that some maximal balanced cliques maybe outputted multiple times if they contain vertices from different sets. To avoid this problem, when a maximal balanced clique  $C$ is explored during the enumeration in $G'_i$, if $C$ contains a vertex $v  \in S_j$, where $j < i$, then $C$ will not be outputted as it has been outputted during the enumeration in $G'_j$. As we can obtain $G'_i$ by scanning    $G$ on the disk once, the I/O complexity of our algorithm is $O(t \cdot \frac{(n+m)}{B})$, where $t$ is the number of partitions and $B$ is the disk block size.


%\stitle{Parallel \kw{MBCE}.} \refalg{fmbcp} can be easily extended to run in parallel. In \refalg{fmbcp}, we explore maximal balanced cliques from each vertex and their neighbors in line 1 (line 2 of \refalg{fmbc}). Since the explorations from different vertices are totally independent, for each $v_i$, we create a new thread to enumerate the maximal balanced cliques related to $v_i$ as \refalg{fmbcp}. All the maximal cliques are enumerated when all the threads are terminated. The correctness of the algorithm can be proved similar to \refalg{fmbc}.

